La conjecture de Casas Alvero pour les degr\'es $5p^{e}$

According to Casas Alvero conjecture, if a one variable polynomial of degree $n$ over a field of characteristic 0 is not prime with each of the $n-1$ first derivees, then it is of the form $c (X-r)^{n}$. Let $p$ be a prime number and an integer $e$, the conjecture is showed to be true for polynomials of degree $p^{e}, 2p^{e}, 3p^{e} (p neq 2) and 4p^{e} (p neq 3,5, 7) $. In this work we show that the conjecture is true for polynomials of degree $5p^{e} (p neq 2,3,7,11,131,193,599,3541,8009) $ . It also corrects an error in Draisma and Jong (2011) for the polynomials of degree $4p^{e}$ ----- Selon la conjecture de Casas Alvero, si un polyn\^{o}me \'{a} une variable de degr\'{e} $n$ sur un corps commutatif de caract\'{e}ristique 0 est non premier avec chacune de ses $n-1$ premi\'{e}res d\'{e}riv\'{e}s, alors il est de forme $c(X-r)^{n}$. Soient $p$ un nombre premier et $e$ un entier, la conjecture a \'{e}t\'{e} d\'{e}montr\'{e}e pour les polyn\^{o}mes de degr\'{e} $p^{e},2p^{e}, 3p^{e} (p\neq 2) et 4p^{e} (p\neq 3,5,7)$. Dans ce travail on montre que la conjecture est vrai pour les polyn\^{o}mes de degr\'{e} $5p^{e} (p\neq 2,3,7,11,131,193,599,3541,8009)$. On corrige aussi une erreur dans Draisma et Jong (2011) pour les degr\'{e} $4p^{e}$

==> ENV.TEX <==
%%              ceci est un fichier preambule           %%
%%%%                 MACROS              %%%%%%%%%%%%%%

%\newcommand{\cqfd}{\nolinebreak \hspace*{5mm} \rule{2mm}{2mm}}
%\newcommand{\f}{\nolinebreak \hspace*{5mm} \rule{1mm}{1mm}}
%\newcommand{\pre}{{\bf Preuve:}}

\def\R{{\mathbb R}}
\def\Z{{\mathbb Z}}
\def\N{{\mathbb N}}
\def\Q{{\mathbb Q}}
\def\ca{${\cal C}_{\de}^{1}(U)$}
\def\C{{\mathbb C}}
%\def\dfrac{{\displaystyle \frac{#1}{#2}}


%\newcounter{remark}
%\newcommand{\rk}{\addtocounter{remark}{1}\smallskip\par\noindent{\bf Remarque}
%\theremark: \nopagebreak}
%\oddsidemargin12mm
%\evensidemargin12mm

         %%%%%%%% LETTRES GREQUES %%%%%%%%
\newcommand{\ga}{\gamma}
\newcommand{\gr}{nabla}
\newcommand{\Ga}{\Gamma}
\newcommand{\De}{\Delta}
\newcommand{\de}{\delta}
\newcommand{\al}{\alpha}
\newcommand{\la}{\lambda}
\newcommand{\be}{\beta}
\newcommand{\ep}{\varepsilon}
\newcommand{\vfi}{\varphi}
\newcommand{\Om}{\Omega}
\newcommand{\si}{\sigma}
\newcommand{\om}{\omega}
         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

         %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newtheorem{df}{D\'efinition}
\newtheorem{thm}{Th\'eor\`eme}
\newtheorem{lem}{Lemme}
\newtheorem{pro}{Proposition}
\newtheorem{rem}{Remarque}
\newtheorem{cor}{Corollaire}

\newcommand{\sev}[2]{\put(#1,-#1){\line(0,1){#2}}
\put(#1,#1){\line(-1,0){#2}}
\put(-#1,#1){\line(0,-1){#2}}
\put(-#1,-#1){\line(1,0){#2}}
\put(#1,0){\line(-1,1){#1}}
\put(0,#1){\line(-1,-1){#1}}
\put(-#1,0){\line(1,-1){#1}}
\put(0,-#1){\line(1,1){#1}} }

\newcommand{\dfrac}[2]{\displaystyle{\frac{#1}{#2}}}


\newcommand{\opdirect}[1]{\overlay{\hbox{\hspace{4.15mm}$^{\hbox{\circle{12}}}$}}{#1}}


\newenvironment{changemargin}[2]{\begin{list}{}{%
\setlength{\topsep}{0pt}%
\setlength{\leftmargin}{0pt}%
\setlength{\rightmargin}{0pt}%
\setlength{\listparindent}{\parindent}%
\setlength{\itemindent}{\parindent}%
\setlength{\parsep}{0pt plus 1pt}%
\addtolength{\leftmargin}{#1}%
\addtolength{\rightmargin}{#2}%
}\item }{\end{list}}

\newcommand{\emline}[6]{
      \put(#1,#2){\special{em:point #1#3}}%
      \put(#4,#5){\special{em:point #1#6}}%
      \special{em:line #1#3,#1#6}}

